Smooth normal forms for integrable hamiltonian systems near a focus-focus singularity

We prove that completely integrable systems are normalisable in the C infinity category near focus-focus singularities.

==> macro.tex <==
% macros Vu Ngoc San (anglais)

\newlength{\Taille}

%requires package amsmath
\RequirePackage{amsmath}
%begin{latexonly}
%\renewcommand{\textup}[1]{\text{\textit{\emph{#1}}}}
%end{latexonly}
\newcommand{\dessus}{\genfrac{}{}{0pt}{}} % pour mettre deux trucs l'un
                                          % dessus l'autre, sous
                                          % AMSmath, a la place de
                                          % \atop: $\dessus{A}{B}$

% pour annoncer une prépub de l'IF: \prepub{605}{2005}
\newcommand{\prepub}[2]{\vskip 1cm
  \begin{center}
    { \large Prépublication de l'Institut Fourier
      n$^{\textrm{\underline{o}}}$~#1 (#2)}
    \texttt{http://www-fourier.ujf-grenoble.fr/prepublications.html}
  \end{center}
  \vskip 1cm}
%
\newcommand{\dx}{\partial_x}
\newcommand{\dy}{\partial_y}
\newcommand{\dt}{\partial_t}
\newcommand{\dz}{\partial_z}
\newcommand{\dxi}{\partial_\xi}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ddt}{\frac{d}{dt}}
\newcommand{\lie}{\mathcal{L}}
\newcommand{\crochet}[1]{\langle{#1}\rangle}
\newcommand{\pscal}[2]{\langle #1,#2\rangle}
%\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\formel}[1]{[\![#1]\!]}
\newcommand{\ham}[1]{\mathcal{X}_{#1}}
\newcommand{\Lie}[1]{\mathfrak{#1}}
\newcommand{\ad}[1]{{\operatorname{ad}}_{#1}}
\newcommand{\Ad}[1]{{\operatorname{Ad}}_{#1}}
\newcommand{\Aut}{\mathop{\operatorname{Aut}}\nolimits}
\newcommand{\fourier}{\mathcal{F}_h}
\newcommand{\fouriero}{\mathcal{F}}
\newcommand{\re}{\mathop{\mathfrak{R}}\nolimits}
\newcommand{\im}{\mathop{\mathfrak{I}}\nolimits}
%\newcommand{\mbold}[1]{\mbox{\boldmath{$#1$}}}
\newcommand{\mbold}[1]{\textnormal{\boldmath{$#1$}}}

\newcommand{\phy}{\varphi}
\newcommand{\epsi}{\varepsilon}
\newcommand{\bep}{\mbold{\epsilon}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\om}{\omega}
\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}

\newcommand{\ssi}{\Longleftrightarrow}
\newcommand{\impliq}{\Rightarrow}
\newcommand{\fleche}{\rightarrow}
\newcommand{\inject}{\hookrightarrow}
\newcommand{\restr}{\upharpoonright}
\newcommand{\bigrestrs}[1]{\left.#1\right|\hspace{-7.22pt}\upharpoonright}
\newcommand{\bigrestrr}[1]{\left.#1\makebox[0ex]{\hspace{3.7pt}$\upharpoonright$}\right|}
\newcommand{\trsp}{\raisebox{.6ex}{${\scriptstyle t}$}}
\newcommand{\limi}[1]{\displaystyle \lim_{#1}}
\newcommand{\tr}{\mathop{\operatorname{tr}}\nolimits}
\newcommand{\rem}[1][$\!\!$]{\noindent {\sl ${\mathcal{R}}$emark #1. }}
\newcommand{\egdef}{\stackrel{\mathrm{def}}{=}}
% \newcommand{\rond}[1]{\settoheight{\hauteur}{$#1$}\raisebox{\hauteur}{$\scriptscriptstyle\,\,\circ$}\hspace{-1ex}{#1}}

\newcommand{\rond}[1]{\accentset{\circ}{#1}}
% requires \usepackage{accents}



%\newcommand{\flechemap}[1]{
%        \settowidth{\Taille}{\mbox{$ ~ #1 ~$}}
%        \stackrel{ ~ #1 ~ }{
%        \rule{\the\Taille}{0.1ex}\raisebox{-.5ex}{$\!\fleche$}}}
%\newcommand{\Flechebas}[1]{\left\Downarrow \begin{array}{l} ~ \\ #1 \\ ~
%        \end{array}\right.}
%\newcommand{\flechediagbas}[1]{\begin{array}{rl}
%       \mathbf{\diagdown} & \\
%       #1 & \hspace{-0.8em}\searrow \end{array}}
\newcommand{\flechediagbas}[1]{%
        \settowidth{\unitlength}{\mbox{$ ~ #1 ~$}}%
        \begin{array}{r}\begin{picture}(0.1,0.5)(0,0)%
        \put(-0.4,0.5){\vector(1,-1){1}}%
        \end{picture}\\ #1 \end{array}}
\newcommand{\flechebas}[1]{%
  \settoheight{\unitlength}{\mbox{$#1$}}%
  \settowidth{\Taille}{\mbox{~${\scriptstyle #1}$}}%
  \addtolength{\unitlength}{4ex}%
  \begin{picture}(0,1)
    \put(0,1){\vector(0,-1){1}}
    \put(0,0.5){\makebox(0,0){${\scriptstyle #1}$ \hspace{\the\Taille}}}
  \end{picture}}
\newcommand{\flechehaut}[1]{%
  \settoheight{\unitlength}{\mbox{$#1$}}%
  \settowidth{\Taille}{\mbox{~${\scriptstyle #1}$}}%
  \addtolength{\unitlength}{4ex}%
  \begin{picture}(0,1)
    \put(0,0){\vector(0,1){1}}
    \put(0,0.5){\makebox(0,0){\hspace{\the\Taille}${\scriptstyle #1}$ }}
  \end{picture}}
\newcommand{\flechedroite}[1]{%
  \settowidth{\unitlength}{\mbox{$#1$}}
  \settoheight{\Taille}{\mbox{${\scriptstyle #1}$}}
  \addtolength{\Taille}{1ex}
  \addtolength{\unitlength}{4ex}
  \raisebox{0.5ex}{%
  \begin{picture}(1,0)
    \put(0,0){\vector(1,0){1}}
    \put(0.5,0){\makebox(0,0){${\scriptstyle #1}$ \vspace{\the\Taille}}}
  \end{picture}}}
\newcommand{\flechegauche}[1]{%
  \settowidth{\unitlength}{\mbox{$#1$}}
  \settoheight{\Taille}{\mbox{${\scriptstyle #1}$}}
  \addtolength{\Taille}{1ex}
  \addtolength{\unitlength}{4ex}
  \begin{picture}(1,0)
    \put(1,0){\vector(-1,0){1}}
    \put(0.5,0){\makebox(0,0){${\scriptstyle #1}$ \vspace{\the\Taille}}}
  \end{picture}}
\newcommand{\vecteur}[1]{%
  \settowidth{\unitlength}{\mbox{$#1$}}%
  \addtolength{\unitlength}{-0.5ex}%
  \settoheight{\Taille}{\fbox{$#1$}}%
  \raisebox{\Taille}%
  {\begin{picture}(0,0)%
      \put(0,0){\vector(1,0){1}}%
    \end{picture}}\!#1}
% cette commande peut remplacer \overrightarrow, qui ne marche pas
% bien (??) en 11pt. Attention,produit une erreur si la fleche est
% petite !!! (utiliser \vec alors)
\newcommand{\cutevector}[1]{%
  \,\settowidth{\unitlength}{\mbox{$#1$}}%
  \addtolength{\unitlength}{-1.3ex}%
  \settoheight{\Taille}{\mbox{$#1$}}%
  \addtolength{\Taille}{0.5ex}%
  {\raisebox{\Taille}{\begin{picture}(0,0)
        \put(0,0){\line(1,0){1}}
        \put(1,0){\raisebox{-0.35pt}{\makebox(0,0){${\scriptstyle
                \rightarrow}$}}}
      \end{picture}}\!#1}%
  \addtolength{\Taille}{0.4ex}\rule{0cm}{\Taille}}
% devrait faire a peu pres la meme chose, mais sans erreur si trop
% petit (mais sans etre plus beau que \vec: ca va depasser)
\newcommand{\cutevectorbis}[1]{\makebox[0.6ex][l]{$#1$}\settowidth{\unitlength}{\mbox{$#1$}}\addtolength{\unitlength}{-0.5ex}\settoheight{\Taille}{\mbox{$#1$}}\addtolength{\Taille}{0.4ex}\raisebox{\Taille}{\makebox[\unitlength][l]{\hrulefill\raisebox{-0.35ex}{$\!{\scriptstyle
      \rightarrow}$}}}}
\newcommand{\tinyvector}[1]{\cutevector{\mbox{${\scriptscriptstyle #1}$}}}


\newcommand{\cqfd}{\hfill $\square$\par\vspace{1ex}}
\newcommand{\finex}{$\diamond$}
\newcommand{\finrem}{\hfill $\oslash$}
\newcommand{\dens}{\Omega_{\frac{1}{2}}}
\newcommand{\Cinf}{C^\infty}
\newcommand{\COT}[1]{T^* #1 \setminus\{0\}}
\newcommand{\intint}{\int\!\!\!\int}
\newcommand{\gener}[1]{\langle #1 \rangle}
\newcommand{\ind}{\mathop{\operatorname{Ind}}\nolimits}
\newcommand{\coker}{\mathop{\operatorname{Coker}}\nolimits}
%\newcommand{\im}{\text{\it {\em Im }}}
\newcommand{\ssub}{\sigma_{\mathrm{sub}}}
%\newcommand{\spec}{\text{\it {\em Spec }}}

%a definir si pas amstex:
%\def\mod{\mathop{\operatorname{mod}}\nolimits}

\newcommand{\h}{\hbar}
\newcommand{\oh}{O(h^\infty)}
\newcommand{\ohb}{O(\hbar^\infty)}

\newcommand{\fio}{Fourier integral operator}
%\newcommand{\opifs}{op\'erateurs int\'egraux de Fourier}
\newcommand{\pdo}{pseudo\-differential operator}
%\newcommand{\opds}{op\'erateurs pseudo-diff\'erentiels}
%\newcommand{\ot}{op\'erateur de Toeplitz}
%\newcommand{\ots}{op\'erateurs de Toeplitz}
%\newcommand{\diffeo}{diff\'eo\-mor\-phis\-me}
%\newcommand{\diffeos}{diff\'eo\-mor\-phis\-mes}
%\newcommand{\bicas}{bicaract\'eristiques}
%\newcommand{\ma}{math\'ematiques}
%\newcommand{\ana}{analyse}
%\newcommand{\geo}{g\'eom\'etrie}
\newcommand{\das}{asymptotic expansion}
\newcommand{\cdv}{Colin de Verdi\`ere}
%\newcommand{\bsur}{bien-s\^ur}
\newcommand{\cis}{completely integrable system}
\newcommand{\mi}{microlocal}
\newcommand{\schr}{Schr\"o\-ding\-er}
\newcommand{\BS}{Bohr-Sommer\-feld}
\newcommand{\ouf}{\vspace{3mm}}
\newcommand{\semicla}{semi-classical}

\newcommand{\AAAA}{\fbox{** \`A COMPL\'ETER **}}

\newcommand{\warning}{\raisebox{-2ex}{\includegraphics[height=6ex]{warning}}}

% Symboles AMS
% version precedente: mettre ymath si disponible. Sinon, Bbb
% deja fait dans barre.sty:
\newcommand{\RM}{\mathbb{R}}
\newcommand{\ZM}{\mathbb{Z}}
\newcommand{\QM}{\mathbb{Q}}
\newcommand{\NM}{\mathbb{N}}
\newcommand{\CM}{\mathbb{C}}

\newcommand{\T}{\mathbb{T}}

\newcommand{\PM}{\mathbb{P}}
\newcommand{\LM}{\barre{L}}

\newcommand{\B}{\mathcal{B}}
\newcommand{\F}{\mathcal{F}}
%\newcommand{\K}{\mathcal{K}}
\newcommand{\A}{\mathcal{A}}

\renewcommand{\O}{\mathscr{O}}

\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}

%\renewcommand{\thesection}{\Roman{section}}

\newcommand{\scratch}[1]{\textsl{[\textcolor{blue}{#1}]}}

\newcommand{\mypart}[1]{\part{\fbox{\mbox{\sf\em{#1}}}}}

\newcommand{\theor}{Theorem}
\newcommand{\defin}{Definition}
\newcommand{\lemma}{Lemma}
\newcommand{\remar}{Remark}
\newcommand{\exemp}{Example}
\newcommand{\corol}{Corollary}
\newcommand{\propo}{Proposition}
\newcommand{\demon}{Proof}
\newcommand{\probl}{Problem}
\newtheorem{theo}{\theor}[section]
\newtheorem{theo*}{\theor}
% ancienne version (jusqu'au 22 mai 2003:)
% \newtheorem{defi}{\defin}[section]
% maintenant on numerote tout sequentiellement
\newtheorem{defi}[theo]{\defin}
\newtheorem{defi*}[theo*]{\defin}
\newtheorem{prop}[theo]{\propo}
\newtheorem{lemm}[theo]{\lemma}
\newtheorem{coro}[theo]{\corol}
\newtheorem{conj}[theo]{Conjecture}
%\newtheorem{prob}{Problem}[section]
\newtheorem{prob}{\probl}[section]

\newcommand{\demons}[1][$\!\!$]{\noindent\textbf{\demon\ }\textsl{#1}\textbf{.}~}
%\newtheorem{rema}{\remar}[section]

%ancienne version (changee 08/07/98):
%\newenvironment{rema}[1][{$\!\!$}]
%{\noindent$\ulcorner${\sl${\mathcal{R}}$emark #1.~}}
%{\noindent$\lrcorner$
%
%}

% anciemmen version (avant 20 mai 2003):
% \newcounter{rema}[section]
% \setcounter{rema}{0}
% \def\therema{\thesection.\arabic{rema}}

% \newenvironment{rema}
% {\par\vspace{1ex}\refstepcounter{rema}%
% \noindent\textbf{\remar~\therema}. }
% {\penalty 500\hfill\mbox{$\triangle$}\par\vspace{1ex}}
\newenvironment{rema}
{\par\vspace{1ex}\refstepcounter{theo}%
\noindent\textbf{\remar~\thetheo} }
{~\hfill\mbox{$\triangle$}\par\vspace{1ex}}

\newenvironment{exem}
{\par\vspace{1ex}\refstepcounter{theo}%
\noindent\textbf{\exemp~\thetheo} }
{\penalty 500\hfill\mbox{$\bigstar$}\par\vspace{1ex}}

%numerotation des equations
%\def\theequation{\thesection.\arabic{equation}}
%\@addtoreset{equation}{section}

% environement ``hypothese'':
\newcounter{hypo}
\setcounter{hypo}{0}
\def\thehypo{\textbf{\textup{(H\arabic{hypo})}}}

\newenvironment{hypo}
{\refstepcounter{hypo}%
\begin{center}\thehypo.\hfill\begin{minipage}{.9\linewidth}}
{\end{minipage}\end{center}}

% demo
\newenvironment{demo}[1][$\!\!$]
{\demons[#1]\ }
{\cqfd}

%environement liste continue (enumerate avec continuite des numeros)
\newcounter{listcont}
\setcounter{listcont}{0}
\def\thelistcont{\arabic{listcont}}

\newenvironment{listcont}
{%\refstepcounter{listcont}%
\begin{enumerate}\setcounter{enumi}{\thelistcont}}
{\end{enumerate}\setcounter{listcont}{\arabic{enumi}}}


% pour la typographie des adresses URL
\newcommand{\ellastiq}{\hspace{0pt plus 0.5ex}}

%la convention standard pour les footnotes est debile en math:
\renewcommand{\thefootnote}{(\arabic{footnote})}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: nil
%%% End: 

